StatBot.Swiss: Bilingual Open Data Exploration in Natural Language

The potential for improvements brought by Large Language Models (LLMs) in Text-to-SQL systems is mostly assessed on monolingual English datasets. However, LLMs' performance for other languages remains vastly unexplored. In this work, we release the StatBot.Swiss dataset, the first bilingual benchmark for evaluating Text-to-SQL systems based on real-world applications. The StatBot.Swiss dataset contains 455 natural language/SQL-pairs over 35 big databases with varying level of complexity for both English and German. We evaluate the performance of state-of-the-art LLMs such as GPT-3.5-Turbo and mixtral-8x7b-instruct for the Text-to-SQL translation task using an in-context learning approach. Our experimental analysis illustrates that current LLMs struggle to generalize well in generating SQL queries on our novel bilingual dataset.

==> figures/intentresultstable.tex <==
\begin{tabular}{c|rrr|rrr|rrr}
         & \multicolumn{3}{c|}{\textbf{Dev}}                                                                                  & \multicolumn{3}{c|}{\textbf{Test}}                                                                                 & \multicolumn{3}{c}{\textbf{Cross-Evaluation}}                                                                                                                                                       \\
         & \multicolumn{1}{c}{\textbf{English}} & \multicolumn{1}{c}{\textbf{German}} & \multicolumn{1}{c|}{\textbf{Overall}} & \multicolumn{1}{c}{\textbf{English}} & \multicolumn{1}{c}{\textbf{German}} & \multicolumn{1}{c|}{\textbf{Overall}} & \multicolumn{1}{c}{\textbf{English}}                            & \multicolumn{1}{c}{\textbf{German}}                             & \multicolumn{1}{c}{\textbf{Overall}}                            \\ \hline
\begin{tabular}[c]{@{}c@{}}\textbf{Language}\\ \textbf{Detection}\end{tabular}   & \multicolumn{1}{l}{}                 & \multicolumn{1}{l}{}                & \multicolumn{1}{l|}{}                 & \multicolumn{1}{l}{}                 & \multicolumn{1}{l}{}                & \multicolumn{1}{l|}{}                 & \multicolumn{1}{l}{}                                            & \multicolumn{1}{l}{}                                            & \multicolumn{1}{l}{}                                            \\ \hline
\textit{LangDetect}           & 0.95                               & 1.00                             & 0.98                                & 1.00                                & 1.00                               & 1.00                                 & 0.99                                                          & 1.00                                                           & 0.99                                                          \\
\textit{LangID}               & 1.00                               & 1.00                               & 1.00                                & 1.00                                & 1.00                               & 1.00                                 & 0.99                                                          & 1.00                                                           & 0.99                                                          \\
\textit{Rocchio}              & 1.00                               & 1.00                               & 1.00                                & 1.00                                & 1.00                               & 1.00                                 & 1.00                                                          & 1.00                                                           & 1.00                                                          \\
\textit{Ensemble}             & 1.00                               & 1.00                               & 1.00                                & 1.00                                & 1.00                               & 1.00                                 & \textbf{1.00}                                                          & \textbf{1.00}                                                           & \textbf{1.00}                                                          \\ 
\hline
\hline

\begin{tabular}[c]{@{}c@{}}\textbf{Table}\\ \textbf{Classification}\end{tabular} &                                      &                                     &                                       &                                      &                                     &                                       &                                                                 &                                                                 &                                                                 \\ 
\hline
\textit{BM25 (r@1)}           & 0.95                               & 0.97                              & 0.96                                & 0.90                               & 0.93                              & 0.92                                & \begin{tabular}[c]{@{}r@{}}0.93\\ ($\pm$ 0.13)\end{tabular} & \begin{tabular}[c]{@{}r@{}}\textbf{0.90}\\ ($\pm$ 0.14)\end{tabular} & \begin{tabular}[c]{@{}r@{}}\textbf{0.91}\\ ($\pm$ 0.11)\end{tabular} \\
\textit{BM25 (r@3)}           & 1.00                               & 1.00                              & 1.00                                & 1.00                               & 0.96                              & 0.98                                & \begin{tabular}[c]{@{}r@{}}0.99\\ ($\pm$ 0.05)\end{tabular} & \begin{tabular}[c]{@{}r@{}}0.98\\ ($\pm$ 0.06)\end{tabular} & \begin{tabular}[c]{@{}r@{}}0.99\\ ($\pm$ 0.03)\end{tabular} \\
\textit{BM25 (r@5)}           & 1.00                               & 1.00                              & 1.00                                & 1.00                               & 0.98                              & 0.99                                & \begin{tabular}[c]{@{}r@{}}1.00\\ ($\pm$ 0.00)\end{tabular} & \begin{tabular}[c]{@{}r@{}}0.98\\ ($\pm$ 0.07)\end{tabular} & \begin{tabular}[c]{@{}r@{}}0.99\\ ($\pm$ 0.03)\end{tabular} \\
\hline
\textit{BERT (r@1)}           & 0.90                               & 0.94                              & 0.92                                & 0.92                               & 0.93                              & 0.93                                & \begin{tabular}[c]{@{}r@{}}\textbf{0.94}\\ ($\pm$ 0.21)\end{tabular} & \begin{tabular}[c]{@{}r@{}}0.87\\ ($\pm$ 0.21)\end{tabular} & \begin{tabular}[c]{@{}r@{}}0.90\\ ($\pm$ 0.12)\end{tabular} \\
\textit{BERT (r@3)}           & 1.00                               & 1.00                              & 1.00                                & 1.00                               & 0.96                              & 0.98                                & \begin{tabular}[c]{@{}r@{}}0.99\\ ($\pm$ 0.10)\end{tabular} & \begin{tabular}[c]{@{}r@{}}0.97\\ ($\pm$ 0.10)\end{tabular} & \begin{tabular}[c]{@{}r@{}}0.98\\ ($\pm$ 0.07)\end{tabular} \\
\textit{BERT (r@5)}           & 1.00                               & 1.00                              & 1.00                                & 1.00                               & 0.98                              & 0.99                                & \begin{tabular}[c]{@{}r@{}}0.99\\ ($\pm$ 0.05)\end{tabular} & \begin{tabular}[c]{@{}r@{}}0.98\\ ($\pm$ 0.10)\end{tabular} & \begin{tabular}[c]{@{}r@{}}0.99\\ ($\pm$ 0.05)\end{tabular}
\end{tabular}

==> figures/zero-shot-prompt.tex <==
You are a helpful AI assistant who writes SQL query for a given question. Given the database described by the database schema below, write a SQL query that answers the question.
Do not explain the SQL query.
Return just the query, so it can be run verbatim from your response.
### Database Schema

CREATE TABLE experiment.spatial_unit (
    spatialunit_uid VARCHAR(30) NOT NULL, 
	spatialunit_current_id INTEGER NOT NULL, 
	spatialunit_ontology VARCHAR(30) NOT NULL, 
	name VARCHAR(100) NOT NULL, 
	name_de VARCHAR(100), 
	name_fr VARCHAR(100), 
	name_it VARCHAR(100), 
	country BOOLEAN DEFAULT false NOT NULL, 
	canton BOOLEAN DEFAULT false NOT NULL, 
	district BOOLEAN DEFAULT false NOT NULL, 
	municipal BOOLEAN DEFAULT false NOT NULL, 
	residence_area BOOLEAN DEFAULT false NOT NULL, 
	neighborhood BOOLEAN DEFAULT false NOT NULL, 
	region BOOLEAN DEFAULT false NOT NULL, 
	zone BOOLEAN, 
	spatialunit_hist_id INTEGER, 
	canton_hist_id INTEGER, 
	district_hist_id INTEGER, 
	valid_from DATE, 
	valid_until DATE, 
	CONSTRAINT spatial_unit_pkey PRIMARY KEY (spatialunit_uid)
)
/*
Columns in spatial_unit and 5 examples in each column for high cardinality columns :
spatialunit_uid : 4837_A.ADM3, 5163_A.ADM3, 994_A.ADM3, 5917_A.ADM3, 4309_A.ADM3
spatialunit_current_id : 2309, 1502, 249, 2225, 713
name : Borgnone, Chapelle (Broye), Valeyres-sous-Ursins, Oppikon, Amtsbezirk Oberhasli
name_de : Borgnone, Chapelle (Broye), Valeyres-sous-Ursins, Oppikon, Amtsbezirk Oberhasli
name_fr : Borgnone, Chapelle (Broye), Valeyres-sous-Ursins, Oppikon, Amtsbezirk Oberhasli
name_it : Borgnone, Chapelle (Broye), Valeyres-sous-Ursins, Oppikon, Amtsbezirk Oberhasli
spatialunit_hist_id : 11616, 11038, 15649, 11681, 11390
canton_hist_id : 8, 25, 22, 26, 16
district_hist_id : 10313, 10276, 10252, 10186, 10106
valid_from : 2001-04-13, 1979-01-01, 2006-01-01, 1993-01-01, 2001-01-01
valid_until : 2009-12-31, 2015-12-31, 2017-12-31, 2000-12-31, 2018-12-31
*/




CREATE TABLE experiment.stock_vehicles (
	uid BIGINT NOT NULL, 
	spatialunit_uid VARCHAR(100), 
	vehicle_type VARCHAR(50), 
	year INTEGER, 
	amount INTEGER, 
	fuel_type VARCHAR(50), 
	CONSTRAINT stock_vehicles_pk PRIMARY KEY (uid), 
	CONSTRAINT stock_vehicles_spatial_unit_spatialunit_uid_fk FOREIGN KEY(spatialunit_uid) REFERENCES experiment.spatial_unit (spatialunit_uid)
)
/*
Columns in stock_vehicles and 5 examples in each column for high cardinality columns :
uid : 1601067, 1601107, 1601232, 1601065, 1601108
spatialunit_uid : 3202_A.ADM3, 2784_A.ADM3, 5913_A.ADM3, 4107_A.ADM3, 628_A.ADM3
year : 2019, 2014, 2016, 2017, 2013
amount : 407, 453, 4407, 713, 7
fuel_type : Diesel-electric: Normal-hybrid, Gas (mono- and bivalent), Hydrogen, Diesel, Benzine
*/

/*
Column name, Column discription, Example values
vehicle_type, Vehicle type, passenger_cars,trailers,motorcycles
amount, Amount of vehicles, 0,2,240
fuel_type, Fuel type, Hydrogen,Electric,Diesel-electric: Normal-hybrid
*/

   
    ### Question: 
    What was the proportion of electric vehicles in Geneva in 2010?
    ### SQL query:


==> sections/intentdetector.tex <==
Our Intent Detector module aims to identify which dataset contains the information a user wishes to search for, given an input natural language query. For example, with the query ``How many electric vehicles were there in Basel in 2019?'', the Intent Detector would return the table \texttt{stock\_vehicles}, which can then be forwarded to the Text-to-SQL engine.

In our data model, we consider each table as a heterogeneous unit, with disparate data that cannot be joined by an SQL query due to the inhomogeneity of the source data. Thus, we use database tables as the target for the user's intent. We can model this in two ways: as either a retrieval task, where tables are considered as documents to be retrieved by the input query; or as a classification task, where each table represents a single class.

We found that, similarly to other systems using Large Language Models for data discovery \cite{solo}, it quickly becomes infeasible to use a prompt-based LLM on a larger-scale retrieval task such as this: as the data size grows, a textual description of the task scales concurrently, quickly overrunning the model's limits on token input size. Thus, it is necessary to provide an initial information-filtering step before performing more fine-grained retrieval with a Large Language Model. 

As such, similarly to \cite{tableqa}, we compare two systems for detecting intent: a retrieval-modelled BM25 system \cite{bm25main}, and BERT \cite{bertmain} (with \texttt{bert-base-multilingual-cased}) as a table classifier. Our results (Table~\ref{tab:intentresults}) show that both approaches perform well, with 90+\% \textit{recall@1}, and near-perfect retrieval on the \textit{recall@3} test. In contrast to similar approaches \cite{tableqa}, which show that BERT significantly outperforms BM25, we find that for our dataset, which is both closed-domain and smaller in size, both approaches perform similarly well. We discuss these results in more detail in Section~\ref{sec:intentresults}. 

\subsubsection{Training Data Preparation}

For BM25, we use the \textit{table-as-a-document} approach to prepare the training and test data. We derive the document content for each table from three different sources:

\begin{itemize}
    \item A \textbf{metadata table}, containing descriptive information about each table, such as a textual description, the data language (English or German), natural language column titles, and column types (\textit{categorical} or \textit{numerical}). For instance, the entry for the table \texttt{stock\_vehicles} is shown in Figure~\ref{fig:metadatastockvehicles}.
    \item A set of \textbf{example queries}, for each table, ranging between 8-30 queries per table, for a total of 491. The language of these example queries was chosen to match the language of the data contained within the table, with 42\% of the queries being English, and the remainder German.
    \item The \textbf{categorical values} contained within the database table itself, such as, for the column “Citizenship”, we extracted the values “Swiss Citizen” and “Foreign National”.
\end{itemize}

\begin{figure}
    \centering
    \fbox{\begin{minipage}{20em}
        \textbf{Name:} \texttt{stock\_vehicles}

        \textbf{Language:} English
        
        \textbf{Title:} Stock of road vehicles by municipality, as of 2010.
        
        \textbf{Description:} This dataset presents the annual stock of road vehicles by municipality, vehicle group (passenger cars, passenger transport vehicles, material transport vehicles, agricultural vehicles, industrial vehicles, motorbikes, trailers) and fuel since 2010.

        \textbf{Columns:} Vehicle Type, Fuel Type, Number of Vehicles
    \end{minipage}}
    \caption{The metadata table entry for \texttt{stock\_vehicles}}
    \label{fig:metadatastockvehicles}
\end{figure}

We combine this data as follows: the table description, name and column titles from the metadata table, $\mathcal{M}_t$, are concatenated; next, for each categorical column in the table, $\mathcal{C}_t$, the unique values, $\mathcal{V}_{t,c}$, are then appended to the document. In addition, we append each table's training queries, $\mathcal{Q}_t$, to the table document. Thus, our document corpus can be represented by:

$$
\mathcal{D}_t = \mathcal{M}_t \cup \bigcup_{c \in \mathcal{C}_t} \mathcal{V}_{t,c} \cup \mathcal{Q}_t
$$

For the input to our BM25 system, we pre-process these documents using stemming, accent normalization, and stopword removal to form a bag-of-words for each table. For stemming, we use the Snowball Stemmer \cite{snowball} via NLTK \cite{nltk} due to its multilingual capabilities, which cover our target languages.

For BERT, we model the task as a classification problem, and label each example query with its corresponding table, and pre-process each query using the supplied BERT tokenizer. The results of each of these systems is presented in Section~\ref{sec:intentresults}.

==> sections/intentresults.tex <==
\begin{table*}[t]
    \def\arraystretch{1.3}
    \centering
    \small
    \input{figures/intentresultstable}
    \caption{Results of the Intent Detection component. Scores for the Language Detection component are the raw classification accuracy (top part). Scores for the Table Classification task are reported as recall at 1, 3 and 5 (\textit{r@1}, \textit{r@3} and \textit{r@5}) (bottom part). The Train/Dev/Test split was 70\%/10\%/20\% for this evaluation, and results are for a single run with the final model. For the cross-evaluation results, we use 10-folds over the average of 10 random permutations of the entire query set, with error ranges in parenthesis displaying the variance over the 100 models.}
    \label{tab:intentresults}
\end{table*}

We evaluate both BERT and BM25 on a set of 491 queries, each labelled with their corresponding data table. We split these queries on a per-table basis, taking 70\% of the queries for each table for training, 10\% for development and 20\% for testing. In addition, we also perform 10-fold cross-validation over the entire query set, for 10 random permutations of the set.

\subsubsection{Language Detection}

As our BM25 implementation requires the language of the input query to be known, we also utilize a Language Detection module as part of the retrieval process. To detect the language of an input query, we use an ensemble classifier, comprising two out-of-the-box language detectors and one custom Rocchio (nearest centroid) classifier \cite{introtoIR}, trained on data specific to this task. Our ensemble classifier takes the majority vote from all of the three classifiers to select a query language, which has been shown to be a reliable method for language detection on short texts \cite{langidensemble}.

For the out-of-the-box language detectors, we use LangID \cite{langid} and LangDetect \cite{langdetect}. Our custom Rocchio classifier builds a TF-IDF (Term Frequency - Inverse Document Frequency) vector for each table from the table document $\mathcal{D}_t$ (as described in Section~\ref{sec:intentdetector}) and then derives an average centroid vector for each language, $V_l$ using these table vectors, where $T_l$ is the set of tables in a language $l$, $w$ represents each word token from a document, and $t$ is a table:

$$
V_l = \frac{\sum_{t \in T_l} \sum_{w \in \mathcal{D}_t} \text{\textsc{tfidf}}(w,t)}{|T_l|}
$$

Language classification is then performed by similarly vectorizing the input query and using cosine similarity to determine the most similar language vector.

The accuracy of these systems is shown in Table~\ref{tab:intentresults}. LangID and LangDetect were seen to make occasional mistakes on some input queries, whereas our domain-specific Rocchio classifier achieves 100\% accuracy on this task. As our Rocchio classifier may run the risk of generalizing less optimally, we combine all three into an ensemble classifier, which we believe should remedy the deficiencies of both of these methods, that achieves 100\% accuracy on our query set.

\subsubsection{Table Classification}

Given an input query and its detected language, we use BM25 to rank each data table according to its relevance. By treating the pre-processed bag-of-words for each table as a document, we calculate the IDF values over the entire training corpus on a per-language basis, which are then used to compute the BM25 weighting for each table, using the standard parameter values of of $k=1.3$ and $b=0.75$.

We noted that, due to the nature of the categorical values of our dataset, some tables would produce a disproportionately large document, such as \texttt{\seqsplit{criminal\_offences\_registered\_by\_police}}, which contains $240$ unique textual values for the \texttt{\seqsplit{offence\_criminal\_code}} column, such as ``Breach of professional confidentiality in research involving human beings - until 2014 Breach of professional confidentiality in medical research'', whereas most tables contain between 4 and 6 unique categorical values of only a few tokens each.

It has been shown that BM25 can fail on such outlier documents \cite{bm25long}, as the document-length factor in BM25 can under-weight all terms within these documents. In our initial error analysis of the development set, we found that tables such as this were never chosen as relevant by our system. As such, we normalize all document lengths to within 2 standard deviations of the mean, as follows, where $\overline{|\mathcal{D}_t|}$ is the mean document length and $\sigma$ is the standard deviation of the distribution of document lengths:

$$
    |\mathcal{D}_t| = 
    \begin{cases}
        \overline{|\mathcal{D}_t|}, & \text{if } \left||\mathcal{D}_t| - \overline{|\mathcal{D}_t|}\right| > 2\sigma \\
        |\mathcal{D}_t|,            & \text{otherwise}
    \end{cases}
$$

We use this pseudo-length as input to BM25, while still retaining all the terms in the document. With this modification, the affected tables were now appropriately ranked, while the remaining ranks remained stable.

For BERT, we use \texttt{\seqsplit{bert-base-multilingual-cased}}, and fine-tune a multi-class classifier on a set of queries labelled with their corresponding table. For training, we base our parameters on similar work on fine-tuning BERT on small datasets \cite{bertsmalldata}. We likewise use a batch size of 32, a learning rate of $2\times 10^{-5}$, dropout of $0.1$, and train for \{100, 200, 300, 500\} steps. We selected a final value of 300 steps based on evaluation on the development set.

\subsubsection{Results}

Both systems perform well in either language, with an average \textit{recall@1} of over 90\% under cross-evaluation, and 99\% \textit{recall@3}. As can be seen in Table~\ref{tab:intentresults}, our BM25 implementation slightly outperforms BERT over both languages combined, while BERT has higher recall in English. Overall, BERT shows a greater disparity in language scores under cross-evaluation, and has a larger variance in both \textit{recall@1} and \textit{recall@3}. In general, this high variance can be primarily attributed to the small training data size, with some tables having as few as 8 queries in total. Nevertheless, average performance across 10$\times$10 folds remains high, and concurs with the test and development set results.

% We make the code for this evaluation publicly available at \footnote{https://github.zhaw.ch/INODE4Statbot-swiss/statbot-intent-detector-evaluation} to facilitate reproducibilty of our results.

We noted during our error analysis that it may be possible in some cases for a query to be answerable by two or more tables. For broad queries, such as ``How many divorces occurred in Switzerland since 2010?'', and where two or more data sources share a conceptual overlap, such as \texttt{\seqsplit{divorces\_duration\_of\_marriage\_age\_classes}} and \texttt{\seqsplit{divorces\_duration\_of\_marriage\_citizenship\_categories}}, the relevant data could be sourced from either table.

Although, for some more complex queries, both systems return a conceptually correct table, but which only contains partial information, and not the exact requested data, such as ``Can you provide the breakdown of the population by different citizenships, different place of the birth and different residentship in the Canton of Obwalden in 2011?''. This query is labeled as \texttt{\seqsplit{resident\_population\_birthplace\_citizenship\_type}}, but both BERT and BM25 return \texttt{\seqsplit{demographic\_balance\_by\_canton}}, which contains citizenship and migration information, but not information about permanent or non-permanent residency status. In both cases the correct table is returned as the second best match, however. Such queries represent the primary source of error for both systems, as can be seen by the low differential between the \textit{recall@3} and \textit{recall@5} scores.

To account for these discrepancies, it would be possible to augment our Text-to-SQL system to attempt to translate the top-3 ranked tables in turn, and, if errors emerge, the next-best table could be chosen. In this manner, our intent detector also functions as an accurate and efficient information filter for large language models.

Our results show that for a narrow-domain task such as this, it is not difficult to design a robust intent detector with minimal training data, using both classical or contemporary methods.


==> sections/relatedwork.tex <==
Regarding Intent Detection -- namely, filtering for relevant tables or documents to be forwarded to a Question-Answering system -- there have been several recent approaches for both a document-based corpus \cite{textqa,denseretrieval}, and heterogeneous databases \cite{tableqa,tapas}. In \cite{tableqa} and \cite{denseretrieval}, the architecture of the system consists of an initial broad pass over a larger data corpus, followed by a more sophisticated QA component operating on this filtered data.
In the development of the Solo data discovery system \cite{solo}, a Retrieval-Augmented Generation approach is explored, which leverages similar broad-scale Intent Detection methods to filter database tables to a small set, before a Large Language Model is used to query this reduced table set.
